Improved Trajectory Reconstruction for Markerless Pose Estimation

Markerless pose estimation allows reconstructing human movement from multiple synchronized and calibrated views, and has the potential to make movement analysis easy and quick, including gait analysis. This could enable much more frequent and quantitative characterization of gait impairments, allowing better monitoring of outcomes and responses to interventions. However, the impact of different keypoint detectors and reconstruction algorithms on markerless pose estimation accuracy has not been thoroughly evaluated. We tested these algorithmic choices on data acquired from a multicamera system from a heterogeneous sample of 25 individuals seen in a rehabilitation hospital. We found that using a top-down keypoint detector and reconstructing trajectories with an implicit function enabled accurate, smooth and anatomically plausible trajectories, with a noise in the step width estimates compared to a GaitRite walkway of only 8mm.

==> tables/geometric_scores.tex <==
\begin{tabular}{llrrrrrr}
\toprule
 &  & $GC_5$ & $GC_{10}$ & $GC_{20}$ & $\mathcal L_\Pi$ & $\mathcal L_{\mathrm{skeleton}}$ & $\mathcal L_{\mathrm{smooth}}$ \\
Keypoints & Method &  &  &  &  &  &  \\
\midrule
\multirow[c]{3}{*}{MMPoseHalpe} & Robust Triangulation & 0.528 & 0.765 & 0.898 & 11.625 & 138.149 & 73.605 \\
 & Explicit Optimization & 0.532 & 0.751 & 0.882 & 10.054 & 29.515 & 37.684 \\
 & Implicit Optimization & \bfseries 0.540 & \bfseries 0.768 & \bfseries 0.900 & \bfseries 9.222 & \bfseries 0.337 & 18.975 \\
 \midrule
\multirow[c]{3}{*}{OpenPose} & Robust Triangulation & 0.326 & 0.614 & 0.806 & 18.579 & 1402.810 & 161.866 \\
 & Explicit Optimization & 0.336 & 0.612 & 0.822 & 10.968 & 27.456 & 38.586 \\
 & Implicit Optimization & 0.357 & 0.613 & 0.823 & 10.301 & 6.207 & \bfseries 17.457 \\
\bottomrule
\end{tabular}

